Benchmarking Commercial Intent Detection Services with Practice-Driven Evaluations

Intent detection is a key component of modern goal-oriented dialog systems that accomplish a user task by predicting the intent of users' text input. There are three primary challenges in designing robust and accurate intent detection models. First, typical intent detection models require a large amount of labeled data to achieve high accuracy. Unfortunately, in practical scenarios it is more common to find small, unbalanced, and noisy datasets. Secondly, even with large training data, the intent detection models can see a different distribution of test data when being deployed in the real world, leading to poor accuracy. Finally, a practical intent detection model must be computationally efficient in both training and single query inference so that it can be used continuously and re-trained frequently. We benchmark intent detection methods on a variety of datasets. Our results show that Watson Assistant's intent detection model outperforms other commercial solutions and is comparable to large pretrained language models while requiring only a fraction of computational resources and training data. Watson Assistant demonstrates a higher degree of robustness when the training and test distributions differ.

==> Benchmarking Commercial Intent Detection Services withPractice-Driven Evaluations (Camera ready_arxiv).pdf/tables/hint3-mcc.tex <==
\begin{table}[!t]
    \centering
    \setlength{\tabcolsep}{0.3em}\resizebox{\linewidth}{!} {%
    \begin{tabular}{l|llll}
    \toprule
    \textbf{}    & {\underline{\textbf{SOFMattress}}} & {\underline{\textbf{Curekart}}} & {\underline{\textbf{Powerplay11}}} & {\underline{\textbf{Average}}}\\ 
    \toprule 
    Watson Assistant & 62.7                & \textbf{65.0}              & 39.1               & \textbf{55.6}\\ \midrule 
    Dialogflow  & \textbf{63.8}                 & 57.8              & 35.3               & 52.3             \\
    RASA          & 52.6                 & 51.1              & 34.0               & 45.9    \\ 
    LUIS          & 58.1                 & 53.9              & 35.9               & 49.3             \\
    Haptik       & 58.8                 & 60.3              & \textbf{42.5}               & 53.8             \\
    BERT     & 61.7                 & 55.3              & 34.7               & 50.6             \\
    \bottomrule
\end{tabular}}
 \caption{\textbf{Maximum Matthews Correlation coefficient (MCC) for commercial solutions on HINT3.} We compute MCC using thresholds from 0.1 to 0.9 on the HINT3 collection. Results for all methods except Watson Assistant are obtained from \cite{Arora2020HINT3RT}.}
 \label{tab:market-hint3-mcc}
\end{table}

==> Benchmarking Commercial Intent Detection Services withPractice-Driven Evaluations (Camera ready_arxiv).pdf/tables/hint3-threshold.tex <==
\begin{table}[h]
    \centering
    \setlength{\tabcolsep}{0.3em}\resizebox{\linewidth}{!} {%
    \begin{tabular}{l|llll}
    \toprule
    \textbf{}    & {\underline{\textbf{SOFMattress}}} & {\underline{\textbf{Curekart}}} & {\underline{\textbf{Powerplay11}}} & {\underline{\textbf{Average}}}\\ 
    \toprule 
WA enhanced & \underline{\textbf{74.0}}                 & \underline{\textbf{86.7}}              & \textbf{60.7}               & \underline{\textbf{73.8}}    \\ \hline
Dialogflow    & 73.2                 & 75.0              & 59.6               & 69.3             \\
RASA          & 69.3                 & 84.1              & 49.1               & 67.5             \\ 
LUIS          & 59.3                 & 72.6              & 48.0               & 60.0             \\
Haptik       & 72.3                 & 80.3              & \underline{66.5}               & 73.0             \\
BERT         & 73.6                 & 83.6              & 58.5               & 71.9             \\
\bottomrule
\end{tabular}}
\caption{\textbf{Maximum In-scope accuracy for commercial solutions on HINT3} over different thresholds from 0.1 to 0.9. Results for all methods except Watson Assistant are obtained from \cite{Arora2020HINT3RT}. WA performances are in bold and best performances are underlined.}
\label{tab:market-hint3-inscope-accuracy}
\end{table}

==> Benchmarking Commercial Intent Detection Services withPractice-Driven Evaluations (Camera ready_arxiv).pdf/tables/market_accuracy.tex <==
\begin{comment}
\begin{table}[h!]
    \centering
    \setlength{\tabcolsep}{.2em}\resizebox{\linewidth}{!} {%
    \begin{tabular}{c >{\centering\arraybackslash}p{1.5cm} >{\centering\arraybackslash}p{1.3cm} >{\centering\arraybackslash}p{1.3cm} >{\centering\arraybackslash}p{1.3cm} >{\centering\arraybackslash}p{1.3cm} >{\centering\arraybackslash}p{1.3cm}}
    \toprule
    & \multicolumn{2}{c}{\underline{\textbf{CLINC150}}} & \multicolumn{2}{c}{\underline{\textbf{HWU64}}} & \multicolumn{2}{c}{\underline{\textbf{BANKING77}}} \\
     (seconds/\%) & Training Time & Accuracy & Training Time & Accuracy & Training Time & Accuracy \\
    \toprule
%   WA classic & 62.53s & 79.3 & 51.12s & 83.4 & 38.46s & 75.2 \\
    WA enhanced & 108.73s & \textbf{86.0} & 49.72s & \textbf{85.8} & 73.19s & \textbf{80.7} \\
    \hline
    RASA & 836.27s & 68.3 & 556.64s & 78.9 & 927.97s & 76.9 \\
    \bottomrule
    \end{tabular}%
    }
    \caption{Accuracy and training time measurements on CLINC150, HWU64 and BANKING77 datasets. Training is performed on the full train sets and result is on the Tfidf-difficult test sets.}
    \label{tab:market-full}
\end{table}
\end{comment}


\begin{table}[!t]
    \centering
    \small
    \setlength{\tabcolsep}{0.2em}\resizebox{\linewidth}{!} {%
    \begin{tabular}{l|cccccc}
    \toprule
    & \multicolumn{2}{c}{\underline{\textbf{SOFMattress}}} & \multicolumn{2}{c}{\underline{\textbf{Curekart}}} & \multicolumn{2}{c}{\underline{\textbf{Powerplay11}}} \\
     & full & subset & full & subset & full & subset \\
    \toprule
    WA classic & 73.6 & 66.2 & 83.2 & 79.9 & 63.3 & 57.1 \\
    WA enhanced & \textbf{74.0} & \textbf{68.4} & \textbf{86.7} & \textbf{85.4} & 60.7 & 57.8 \\
    \hline
    Dialogflow & 73.1 & 65.3 & 75.0 & 71.2 & 59.6 & 55.6 \\
    RASA & 69.2 & 56.2 & 84.0 & 80.5 & 49.0 & 38.5 \\
    LUIS & 59.3 & 49.3 & 72.5 & 71.6 & 48.0 & 44.0 \\
    Haptik & 72.2 & 64.0 & 80.3 & 79.8 & \textbf{66.5} & \textbf{59.2} \\
    BERT  & 73.5 & 57.1 & 83.6 & 82.3 & 58.5 & 53.0 \\
    \bottomrule
    \end{tabular}%
    }
    \vspace{-0.1in}
    \caption{\textbf{In-scope Accuracy on HINT3 using commercial solutions.} We report the in-scope accuracy with a threshold of 0.1 for various intent detection methods. Results for all methods except Watson Assistant (WA) are obtained from \cite{Arora2020HINT3RT}.}
    \label{tab:market-hint3}
\end{table}

\begin{table}[!t]
    \centering
    \small
    \setlength{\tabcolsep}{1em}\resizebox{\linewidth}{!} {%
    \begin{tabular}{l|ccc}
    \toprule
    & {\underline{\textbf{Full}}} & {\underline{\textbf{Subset}}} & {\underline{\textbf{Average}}} \\
     
    \toprule
    WA classic & 73.4 & 67.7 & 70.6 \\
    WA enhanced & \textbf{73.8} & \textbf{70.5} & \textbf{72.2}\\
    \hline
    Dialogflow & 69.2  & 64.0 & 66.6\\
    RASA & 67.4 & 58.4 & 62.9 \\
    LUIS &  59.9 & 54.6 & 57.5\\
    Haptik &73.0 & 67.6 & 70.3\\
    BERT & 71.9 & 64.1 & 68.0\\
    \bottomrule
    \end{tabular}%
    }
    \vspace{-0.1in}
    \caption{\textbf{Average In-scope Accuracy on HINT3 using commercial solutions.}
    We report the average in-scope accuracy across the three datasets with a threshold of 0.1 on Full and Subset versions of the HINT3 collection. Results for all methods except Watson Assistant (WA) are obtained from \cite{Arora2020HINT3RT}.}
    \label{tab:market-hint3-avg}
\end{table}



==> Benchmarking Commercial Intent Detection Services withPractice-Driven Evaluations (Camera ready_arxiv).pdf/tables/open_source_accuracy_difficult.tex <==
\begin{table}[!t]
\centering
\setlength{\tabcolsep}{0.2em}\resizebox{\linewidth}{!} {%
\begin{tabular}{c >{\centering\arraybackslash}p{1.5cm} >{\centering\arraybackslash}p{1.5cm}  >{\centering\arraybackslash}p{1.5cm}}
\toprule
             & \multicolumn{1}{c}{\underline{\textbf{CLINC150}}}           & \multicolumn{1}{c}{\underline{\textbf{HWU64}}}                & \multicolumn{1}{c}{\underline{\textbf{BANKING77}}}            \\
\toprule
%Algorithm     & Difficult subset  & Difficult subset & Difficult subset \\
%\midrule
WA classic           & 79.3      & 83.4      & 75.2                               \\
WA enhanced           & 86.0  & 85.8  & 80.6 \\
\midrule
RASA             & 68.3      & 78.9      & 76.9                               \\
Distilbert-base  & 85.7      & 87.4      & 79.2                               \\
BERT-base        & 87.6     & 87.6      & 81.7                               \\
BERT-large       & \textbf{89.5}  &\textbf{89.2}  & \textbf{83.9}   \\
USE-base          & 81.6      & 83.4      & 74.5                               \\
RoBERTa-base     & 88.4      & 88.5      & 83.8           \\
\bottomrule              
\end{tabular}%

}

    \caption{\textbf{Accuracy on CLINC150, HWU64 and BANKING77 for Watson Assistant (WA), RASA and pretrained LMs}. Models are trained on full train sets and evaluated on Tfidf-difficult test sets.}
    \label{tab:opensource-accuracy-difficult}
\end{table}

==> Benchmarking Commercial Intent Detection Services withPractice-Driven Evaluations (Camera ready_arxiv).pdf/tables/open_source_accuracy_full.tex <==
\begin{table}[!t]
\centering
\setlength{\tabcolsep}{0.2em}\resizebox{\linewidth}{!} {%
\begin{tabular}{c >{\centering\arraybackslash}p{1.5cm} >{\centering\arraybackslash}p{1.5cm}  >{\centering\arraybackslash}p{1.5cm}
>{\centering\arraybackslash}p{1.5cm}}
\toprule
             & \multicolumn{1}{c}{\underline{\textbf{CLINC150}}}           & \multicolumn{1}{c}{\underline{\textbf{HWU64}}}                & \multicolumn{1}{c}{\underline{\textbf{BANKING77}}}       &
             \multicolumn{1}{c}{\underline{\textbf{Average}}}\\
\toprule
%Algorithm    & Full & Full & Full \\
%\midrule
WA classic           & 93.9       & 88.8      & 90.6    & 91.1                                 \\
WA enhanced           & 95.7 &  90.5 &  92.6  & 92.9\\
\midrule
RASA             & 89.4     & 84.9      & 89.9                        & 88.1      \\
Distilbert-base  & 96.3     & 91.7      & 92.1                        & 93.4      \\
BERT-base        & 96.8     & 91.6      & 93.3                        & 93.9      \\
BERT-large       & \textbf{97.1}   & 91.9   & 93.7                 & 94.2      \\
USE-base         & 94.7     & 88.9      & 89.9                        & 91.2     \\
RoBERTa-base     & 97.0      & \textbf{92.1}      & \textbf{94.1}  & \textbf{94.4} \\
\bottomrule              
\end{tabular}%

}
\vspace{-0.1in}
    \caption{\textbf{Accuracy on CLINC150, HWU64 and BANKING77 for Watson Assistant (WA), RASA and pretrained LMs}. Training is performed on the full train sets and evaluation on full test sets.}
    \label{tab:opensource-accuracy-full}
\end{table}

==> Benchmarking Commercial Intent Detection Services withPractice-Driven Evaluations (Camera ready_arxiv).pdf/tables/open_source_difficult.tex <==
\begin{table}[!h]
\centering
\setlength{\tabcolsep}{0.2em}\resizebox{\linewidth}{!} {%
    \begin{tabular}{@{}ccccccc@{}}
     \toprule
     & \multicolumn{6}{c}{\underline{\textbf{CLINC150}}}                                                        \\
%     \midrule
%                 & \multicolumn{6}{c}{\textbf{ Tfidf-difficult test set}}                 \\
     \midrule
     &
      \multicolumn{2}{c}{\textbf{5 ex/class}} &
      \multicolumn{2}{c}{\textbf{30 ex/class}} &
      \multicolumn{2}{c}{full} \\
    \hline
     &
      Training   time &
      Accuracy &
      Training   time &
      Accuracy &
      Training   time &
      Accuracy \\
      \hline
    WA classic            & 0.58  & 54.0    & 0.78  & 69.9 & 1.04  & 79.3  \\
    WA enhanced           & 0.66  & 65.1 & 0.63  & 76.7 & 1.81  & 86.0     \\
    RASA                  & 1.25  & 29.6  & 5.6   & 52.5 & 13.93 & 68.3  \\
    Distilbert-base       & 15.23 & 63.4  & 31.65 & 76.8  & 35.98 & 85.7  \\
    BERT-base             & 29.67 & 64.6  & 61.43 & 81.1 & 71.08 & 87.6   \\
    BERT-large            & 125   & 72.0    & 280   & 85.6  & 270   & 89.5   \\
    USE-base              & 1.63  & 66.6  & 6.5   & 77.5 & 14.73 & 81.6   \\
    RoBERTa-base          & 33    & 70.8  & 85    & 83.7  & 90    & 88.4   \\
     \toprule
                 & \multicolumn{6}{c}{\underline{\textbf{HWU64}}}                                                                         \\
    %  \midrule             
    %              & \multicolumn{6}{c}{\textbf{ Tfidf-difficult test set}}                 \\
     \midrule
     &
      \multicolumn{2}{c}{\textbf{5 ex/class}} &
      \multicolumn{2}{c}{\textbf{30 ex/class}} &
      \multicolumn{2}{c}{full} \\
     \hline
     &
      Training   time &
      Accuracy &
      Training   time &
      Accuracy &
      Training   time &
      Accuracy \\
    \hline 
    WA classic          & 0.39  & 53.9 & 0.59  & 72.3 & 0.85  & 83.4  \\
    WA enhanced         & 0.75  & 62.7 & 0.54  & 80.0    & 0.82  & 85.8   \\
    RASA                & 0.67  & 34.5 & 2.17  & 63.5 & 9.43  & 78.9  \\
    Distilbert-base     & 6.32  & 63.4 & 13.92 & 79.7 & 20.35 & 87.4  \\
    BERT-base           & 12.73 & 61.6 & 27.18 & 82.1  & 39.48 & 87.6  \\
    BERT-large          & 52    & 71.1  & 120   & 85.3  & 175   & 89.2   \\
    USE-base            & 1.2   & 66.3 & 2.46  & 79.8  & 8.92  & 83.4  \\
    RoBERTa-base        & 13    & 64.5  & 40    & 83.9  & 60    & 88.5   \\
     \toprule
                 & \multicolumn{6}{c}{\underline{\textbf{BANKING77}}}                                                                     \\
    %  \midrule             
    %              & \multicolumn{6}{c}{\textbf{ Tfidf-difficult test set}}                 \\
     \midrule
     &
      \multicolumn{2}{c}{\textbf{5 ex/class}} &
      \multicolumn{2}{c}{\textbf{30 ex/class}} &
      \multicolumn{2}{c}{full} \\
    \hline
     &
      Training   time &
      Accuracy &
      Training   time &
      Accuracy &
      Training   time &
      Accuracy \\
    \hline
    WA classic       & 0.38  & 43.2 & 0.49  & 64.5 & 0.64  & 75.2  \\
    WA enhanced      & 0.65  & 49.1 & 0.52  & 69.7 & 1.22  & 80.6  \\
    RASA             & 0.89  & 26.9 & 3.67  & 57.9 & 15.45 & 76.9  \\
    Distilbert-base  & 7.87  & 50.0    & 16.83 & 69.0 & 20.35 & 79.2  \\
    BERT-base        & 15.23 & 48.3 & 32.72 & 73.4 & 38.75 & 81.7  \\
    BERT-large       & 92    & 52.6  & 210   & 75.8  & 175   & 83.9   \\
    USE-base         & 1.33  & 44.5 & 2.95  & 68.6 & 9.47  & 74.5  \\
    RoBERTa-base     & 17    & 57.1  & 42    & 75.7  & 57    & 83.8   \\
    \bottomrule
    \end{tabular}%
    }
    \caption{\textbf{Accuracy and training time (in minutes) comparing Watson Assistant (WA) with RASA and pretrained LMs}. We use $5/30/$all examples per intent on CLINC150, HWU64 and BANKING77 datasets. Results are the on the respective Tfidf-difficult test sets.}
    \label{tab:opensource-difficult}
\end{table}


==> Benchmarking Commercial Intent Detection Services withPractice-Driven Evaluations (Camera ready_arxiv).pdf/tables/open_source_full.tex <==
\begin{table}[!h]
\centering
\setlength{\tabcolsep}{0.2em}\resizebox{\linewidth}{!} {%
    \begin{tabular}{@{}ccccccc@{}}
     \toprule
     & \multicolumn{6}{c}{\underline{\textbf{CLINC150}}}                                                        \\
    %  \midrule
    %              & \multicolumn{6}{c}{\textbf{Full test set}}                          \\
     \midrule
     &
      \multicolumn{2}{c}{\textbf{5 ex/class}} &
      \multicolumn{2}{c}{\textbf{30 ex/class}} &
      \multicolumn{2}{c}{\textbf{full}} \\
    \hline
     &
      Training   time &
      Accuracy &
      Training   time &
      Accuracy &
      Training   time &
      Accuracy \\
      \hline
    WA classic           & 0.58  & 78.1 & 0.78  & 90.3 & 1.04  & 93.9   \\
    WA enhanced          & 0.66  & 83.6 & 0.63  & 92.5 & 1.81  & 95.7   \\
    RASA                 & 1.25  & 53.2 & 5.6   & 79.4  & 13.93 & 89.4  \\
    Distilbert-base      & 15.23 & 82.2  & 31.65 & 93.2 & 35.98 & 96.3  \\
    BERT-base            & 29.67 & 83.8 & 61.43 & 94.7 & 71.08 & 96.8   \\
    BERT-large           & 125   & 87    & 280   & 95.8  & 270   & 97.1 \\
    USE-base             & 1.63  & 83.9 & 6.5   & 92.9  & 14.73 & 94.7  \\
    RoBERTa-base         & 33    & 86.3  & 85    & 95.4  & 90    & 97.0 \\
     \toprule
                 & \multicolumn{6}{c}{\underline{\textbf{HWU64}}}                                                                         \\
    %  \midrule             
    %              & \multicolumn{6}{c}{\textbf{Full test set}}                 \\
     \midrule
     &
      \multicolumn{2}{c}{\textbf{5 ex/class}} &
      \multicolumn{2}{c}{\textbf{30 ex/class}} &
      \multicolumn{2}{c}{\textbf{full}} \\
     \hline
     &
      Training   time &
      Accuracy &
      Training   time &
      Accuracy &
      Training   time &
      Accuracy \\
    \hline 
    WA classic          & 0.39  & 64.1 & 0.59  & 81.4  & 0.85  & 88.8 \\
    WA enhanced         & 0.75  & 71.0 & 0.54  & 86.2  & 0.82  & 90.5 \\
    RASA                & 0.67  & 43.7 & 2.17  & 72.4  & 9.43  & 84.9 \\
    Distilbert-base     & 6.32  & 71.1 & 13.92 & 86.3  & 20.35 & 91.7 \\
    BERT-base           & 12.73 & 70.1 & 27.18 & 87.5  & 39.48 & 91.6 \\
    BERT-large          & 52    & 77.3  & 120  & 89.3  & 175   & 91.9 \\
    USE-base            & 1.2   & 72.5  & 2.46  & 86.3  & 8.92  & 88.9  \\
    RoBERTa-base        & 13    & 71.7  & 40    & 88.8   & 60    & 92.1 \\
     \toprule
                 & \multicolumn{6}{c}{\underline{\textbf{BANKING77}}}                                                                     \\
    %  \midrule             
    %              & \multicolumn{6}{c}{\textbf{Full test set}}    \\
     \midrule
     &
      \multicolumn{2}{c}{\textbf{5 ex/class}} &
      \multicolumn{2}{c}{\textbf{30 ex/class}} &
      \multicolumn{2}{c}{full} \\
    \hline
     &
      Training   time &
      Accuracy &
      Training   time &
      Accuracy &
      Training   time &
      Accuracy \\
    \hline
    WA classic       & 0.38  & 64.2 & 0.49  & 84.7 & 0.64  & 90.6 \\
    WA enhanced      & 0.65  & 69.9 & 0.52  & 87.0 & 1.22  & 92.6 \\
    RASA             & 0.89  & 45.1 & 3.67  & 81.6 & 15.45 & 89.9 \\
    Distilbert-base  & 7.87  & 69.8  & 16.83 & 87.8 & 20.35 & 92.1 \\
    BERT-base        & 15.23 & 68.3 & 32.72 & 88.9 & 38.75 & 93.3  \\
    BERT-large       & 92    & 71.2  & 210   & 89.9  & 175   & 93.7 \\
    USE-base         & 1.33  & 65.3 & 2.95  & 86.8 & 9.47  & 89.9  \\
    RoBERTa-base     & 17    & 75.9  & 42    & 90.4  & 57    & 94.1  \\
    \bottomrule
    \end{tabular}%
    }
    \caption{\textbf{Accuracy and training time (in minutes) comparing Watson Assistant (WA) with RASA and pretrained LMs}. We use $5/30/$all examples per intent on CLINC150, HWU64 and BANKING77 datasets. Results are the on the respective full test sets.}
    \label{tab:opensource-full}
\end{table}




==> Benchmarking Commercial Intent Detection Services withPractice-Driven Evaluations (Camera ready_arxiv).pdf/tables/open_source_time.tex <==
\begin{table}[!t]
\centering
\setlength{\tabcolsep}{0.2em}\resizebox{\linewidth}{!} {%
\begin{tabular}{ccccc}
\toprule
\multirow{2}{*}{\textbf{Algorithm}} & \multirow{2}{*}{\textbf{Resources}} & \textbf{CLINC150}      & \textbf{HWU}           & \textbf{BANKING77}     \\
                           &          &  Training time &  Training time & Training time \\
\toprule
WA classic                     & -      & \textbf{1.04}          & 0.85          & \textbf{0.64}          \\
WA enhanced                     & -      & 1.81          & \textbf{0.82}          & 1.22          \\
\hline
RASA                       & GPU      & 13.93         & 9.43          & 15.45         \\
Distilbert-base            & GPU      & 35.98         & 20.35         & 20.35         \\
BERT-base                  & GPU      & 71.08         & 39.48         & 38.75         \\
BERT-large                 & GPU      & 270           & 175           & 175           \\
USE-base                   & GPU      & 14.73         & 8.92          & 9.47          \\
RoBERTa-base               & GPU      & 90            & 60            & 57            \\
\bottomrule
\end{tabular}%
}
    \caption{\textbf{Training time (in minutes) and resource requirements} for Watson Assistant (WA), RASA and pretrained LMs. Training is performed on full training sets. All methods except for Watson Assistant are trained using a single NVIDIA K80 GPU.}
    \label{tab:opensource-time}
\end{table}

==> Benchmarking Commercial Intent Detection Services withPractice-Driven Evaluations (Camera ready_arxiv).pdf/tables/wa_comparison.tex <==
\begin{table}[!h]
    \centering
    \setlength{\tabcolsep}{0.1em}\resizebox{\linewidth}{!} {%
     \begin{tabular}{l|lllllll}
    \toprule
                 & {\small \textbf{CLINC150}}      & {\small \textbf{HWU64}}        & {\small\textbf{BANKING77}}     & {\small\textbf{SOF}}   & {\small\textbf{Curekart}}      & {\small\textbf{Power}}   & {\small\textbf{Average}}       \\ 
                 & & & & {\small \textbf{Mattress} } && {\small \textbf{play11}} & \\
    \toprule

   Enhanced & \textbf{95.73} & \textbf{90.52} & \textbf{92.59} & \textbf{74.5} & \textbf{86.5} & 60.7          & \textbf{79.0}\\
    Classic   & 93.88          & 88.75          & 90.58          & 73.6          & 83.2          & \textbf{63.3} & 76.3       
    \\ \bottomrule
\end{tabular}}

\caption{\textbf{Accuracy of new generation of Watson Assistant algorithm (Enhanced) compared to previous generation (Classic) across datasets.} Training is performed on the full train sets and testing is done on respective full test sets.}
\label{tab:wa comparison}
\end{table}

==> Benchmarking Commercial Intent Detection Services withPractice-Driven Evaluations (Camera ready_arxiv).pdf/tables/wa_learning_curve.tex <==
\begin{table}[h]
    \centering
    \setlength{\tabcolsep}{0.1em}\resizebox{\linewidth}{!} {%
\begin{tabular}{llllll}
\toprule
& \multicolumn{5}{c}{\underline{\bf CLINC150}}                                                                                                   \\ 
\midrule
& \multicolumn{1}{c}{\bf 5 ex/class}  & \multicolumn{1}{c}{\bf 15 ex/class} &  \multicolumn{1}{c}{\bf 30 ex/class}& \multicolumn{1}{c}{\bf 80 ex/class} & \multicolumn{1}{c}{\bf full} \\ 
\hline
             & Accuracy & Accuracy & Accuracy & Accuracy & Accuracy \\ 
\hline
WA enhanced  &{\bf 65.1} & {\bf 70.9} & {\bf 76.7} & {\bf 81.5} & {\bf 86.0} \\
WA classic   & 54.0      & 65.2     & 69.9     & 74.7     & 79.3    \\
\toprule
& \multicolumn{5}{c}{\underline{\bf HWU64}}                                                                                                        \\ 
\midrule
& \multicolumn{1}{c}{\bf 5 ex/class}  & \multicolumn{1}{c}{\bf 15 ex/class} &  \multicolumn{1}{c}{\bf 30 ex/class}& \multicolumn{1}{c}{\bf 80 ex/class} & \multicolumn{1}{c}{\bf full} \\ 
\hline
             & Accuracy & Accuracy & Accuracy & Accuracy & Accuracy \\ 
\hline
WA enhanced  & {\bf 62.7} & {\bf 75.6} & {\bf 80.0} & {\bf 84.0} & {\bf 85.8}\\
WA classic   & 53.9      & 66.5      & 72.3    & 80.0   & 83.4     \\
\toprule
& \multicolumn{5}{c}{\underline{\textbf{BANKING77}}}                                                                                                        \\
\midrule
& \multicolumn{1}{c}{\bf 5 ex/class}  & \multicolumn{1}{c}{\bf 15 ex/class} &  \multicolumn{1}{c}{\bf 30 ex/class}& \multicolumn{1}{c}{\bf 80 ex/class} & \multicolumn{1}{c}{\bf full} \\ 
\hline
             & Accuracy & Accuracy & Accuracy & Accuracy & Accuracy \\ 
\hline
WA enhanced & {\bf 49.1} & {\bf 60.8} & {\bf 69.7} & {\bf 76.9} & {\bf 80.6}\\
WA classic  & 43.2    & 56.8    & 64.5    & 72.5    & 75.2       \\
\bottomrule
\end{tabular}%
}
    \caption{Comparing performance of Watson Assistant versions (Enhanced and Classic) in various few-shot settings. Table shows accuracy measurements using $5/15/30/80/$all examples per intent on CLINC150, HWU64 and BANKING77 datasets and testing is done on the respective Tfidf-difficult test sets. Best performances are in bold.}
    \label{tab:wa_learning_curve}
\end{table}



==> tables/hint3-mcc.tex <==
\begin{table}[!t]
    \centering
    \setlength{\tabcolsep}{0.3em}\resizebox{\linewidth}{!} {%
    \begin{tabular}{l|llll}
    \toprule
    \textbf{}    & {\underline{\textbf{SOFMattress}}} & {\underline{\textbf{Curekart}}} & {\underline{\textbf{Powerplay11}}} & {\underline{\textbf{Average}}}\\ 
    \toprule 
    Watson Assistant & 62.7                & \textbf{65.0}              & 39.1               & \textbf{55.6}\\ \midrule 
    Dialogflow  & \textbf{63.8}                 & 57.8              & 35.3               & 52.3             \\
    RASA          & 52.6                 & 51.1              & 34.0               & 45.9    \\ 
    LUIS          & 58.1                 & 53.9              & 35.9               & 49.3             \\
    Haptik       & 58.8                 & 60.3              & \textbf{42.5}               & 53.8             \\
    BERT     & 61.7                 & 55.3              & 34.7               & 50.6             \\
    \bottomrule
\end{tabular}}
 \caption{\textbf{Maximum Matthews Correlation coefficient (MCC) for commercial solutions on HINT3.} We compute MCC using thresholds from 0.1 to 0.9 on the HINT3 collection. Results for all methods except Watson Assistant are obtained from \cite{Arora2020HINT3RT}.}
 \label{tab:market-hint3-mcc}
\end{table}

==> tables/hint3-threshold.tex <==
\begin{table}[h]
    \centering
    \setlength{\tabcolsep}{0.3em}\resizebox{\linewidth}{!} {%
    \begin{tabular}{l|llll}
    \toprule
    \textbf{}    & {\underline{\textbf{SOFMattress}}} & {\underline{\textbf{Curekart}}} & {\underline{\textbf{Powerplay11}}} & {\underline{\textbf{Average}}}\\ 
    \toprule 
WA enhanced & \underline{\textbf{74.0}}                 & \underline{\textbf{86.7}}              & \textbf{60.7}               & \underline{\textbf{73.8}}    \\ \hline
Dialogflow    & 73.2                 & 75.0              & 59.6               & 69.3             \\
RASA          & 69.3                 & 84.1              & 49.1               & 67.5             \\ 
LUIS          & 59.3                 & 72.6              & 48.0               & 60.0             \\
Haptik       & 72.3                 & 80.3              & \underline{66.5}               & 73.0             \\
BERT         & 73.6                 & 83.6              & 58.5               & 71.9             \\
\bottomrule
\end{tabular}}
\caption{\textbf{Maximum In-scope accuracy for commercial solutions on HINT3} over different thresholds from 0.1 to 0.9. Results for all methods except Watson Assistant are obtained from \cite{Arora2020HINT3RT}. WA performances are in bold and best performances are underlined.}
\label{tab:market-hint3-inscope-accuracy}
\end{table}

==> tables/wa_comparison.tex <==
\begin{table}[!h]
    \centering
    \setlength{\tabcolsep}{0.1em}\resizebox{\linewidth}{!} {%
     \begin{tabular}{l|lllllll}
    \toprule
                 & {\small \textbf{CLINC150}}      & {\small \textbf{HWU64}}        & {\small\textbf{BANKING77}}     & {\small\textbf{SOF}}   & {\small\textbf{Curekart}}      & {\small\textbf{Power}}   & {\small\textbf{Average}}       \\ 
                 & & & & {\small \textbf{Mattress} } && {\small \textbf{play11}} & \\
    \toprule

   Enhanced & \textbf{95.73} & \textbf{90.52} & \textbf{92.59} & \textbf{74.5} & \textbf{86.5} & 60.7          & \textbf{79.0}\\
    Classic   & 93.88          & 88.75          & 90.58          & 73.6          & 83.2          & \textbf{63.3} & 76.3       
    \\ \bottomrule
\end{tabular}}

\caption{\textbf{Accuracy of new generation of Watson Assistant algorithm (Enhanced) compared to previous generation (Classic) across datasets.} Training is performed on the full train sets and testing is done on respective full test sets.}
\label{tab:wa comparison}
\end{table}

==> tables/wa_learning_curve.tex <==
\begin{table}[h]
    \centering
    \setlength{\tabcolsep}{0.1em}\resizebox{\linewidth}{!} {%
\begin{tabular}{llllll}
\toprule
& \multicolumn{5}{c}{\underline{\bf CLINC150}}                                                                                                   \\ 
\midrule
& \multicolumn{1}{c}{\bf 5 ex/class}  & \multicolumn{1}{c}{\bf 15 ex/class} &  \multicolumn{1}{c}{\bf 30 ex/class}& \multicolumn{1}{c}{\bf 80 ex/class} & \multicolumn{1}{c}{\bf full} \\ 
\hline
             & Accuracy & Accuracy & Accuracy & Accuracy & Accuracy \\ 
\hline
WA enhanced  &{\bf 65.1} & {\bf 70.9} & {\bf 76.7} & {\bf 81.5} & {\bf 86.0} \\
WA classic   & 54.0      & 65.2     & 69.9     & 74.7     & 79.3    \\
\toprule
& \multicolumn{5}{c}{\underline{\bf HWU64}}                                                                                                        \\ 
\midrule
& \multicolumn{1}{c}{\bf 5 ex/class}  & \multicolumn{1}{c}{\bf 15 ex/class} &  \multicolumn{1}{c}{\bf 30 ex/class}& \multicolumn{1}{c}{\bf 80 ex/class} & \multicolumn{1}{c}{\bf full} \\ 
\hline
             & Accuracy & Accuracy & Accuracy & Accuracy & Accuracy \\ 
\hline
WA enhanced  & {\bf 62.7} & {\bf 75.6} & {\bf 80.0} & {\bf 84.0} & {\bf 85.8}\\
WA classic   & 53.9      & 66.5      & 72.3    & 80.0   & 83.4     \\
\toprule
& \multicolumn{5}{c}{\underline{\textbf{BANKING77}}}                                                                                                        \\
\midrule
& \multicolumn{1}{c}{\bf 5 ex/class}  & \multicolumn{1}{c}{\bf 15 ex/class} &  \multicolumn{1}{c}{\bf 30 ex/class}& \multicolumn{1}{c}{\bf 80 ex/class} & \multicolumn{1}{c}{\bf full} \\ 
\hline
             & Accuracy & Accuracy & Accuracy & Accuracy & Accuracy \\ 
\hline
WA enhanced & {\bf 49.1} & {\bf 60.8} & {\bf 69.7} & {\bf 76.9} & {\bf 80.6}\\
WA classic  & 43.2    & 56.8    & 64.5    & 72.5    & 75.2       \\
\bottomrule
\end{tabular}%
}
    \caption{Comparing performance of Watson Assistant versions (Enhanced and Classic) in various few-shot settings. Table shows accuracy measurements using $5/15/30/80/$all examples per intent on CLINC150, HWU64 and BANKING77 datasets and testing is done on the respective Tfidf-difficult test sets. Best performances are in bold.}
    \label{tab:wa_learning_curve}
\end{table}


